Interpreting Dense Retrieval as Mixture of Topics

Dense Retrieval (DR) reaches state-of-the-art results in first-stage retrieval, but little is known about the mechanisms that contribute to its success. Therefore, in this work, we conduct an interpretation study of recently proposed DR models. Specifically, we first discretize the embeddings output by the document and query encoders. Based on the discrete representations, we analyze the attribution of input tokens. Both qualitative and quantitative experiments are carried out on public test collections. Results suggest that DR models pay attention to different aspects of input and extract various high-level topic representations. Therefore, we can regard the representations learned by DR models as a mixture of high-level topics.

==> exp_setup.tex <==

\section{Experimental Setup}

Here we present our experimental settings, including datasets, baselines, and implementation details.

\paragraph{Datasets and Metrics}

\paragraph{Baselines}
We exploit two types of baselines, vector compression methods and retrieval models.
Unsupervised methods include OPQ~\cite{ge2013optimized}. We use Faiss library~\cite{johnson2019billion} to implement those baselines. 
Supervised methods include recently proposed JPQ~\cite{zhan2021jointly}, both of which are also based on PQ. 
DR models include ANCE~\cite{xiong2021approximate} and ADORE~\cite{zhan2021optimizing}. Their output embeddings are of dimension $768$ and are not compressed. All of them utilize negative sampling methods for training as RepCONC.  

\paragraph{Implementation Details}

Here are our model settings.
We build RepCONC based on huggingface transformers~\cite{wolf2019huggingface} and Faiss ANNS library~\cite{johnson2019billion}. The dual-encoders use RoBERTa-base~\cite{liu2019roberta} as the backbone, and the output embedding dimension is 768. Embedding similarity is computed with inner product. For PQ hyper-parameters, $K$ is set to 256, and $M$ is set to 4, 8, 12, 16, 24, 32, and 48. 

Training settings are as follows. 
Most training hyper-parameters are kept the same in both datasets except for batch size due to the limitation of GPU memory. 
Following ADORE~\cite{zhan2021optimizing}, training is in two stages. 
In the first stage where static hard negatives are used, the optimizer is AdamW~\cite{loshchilov2017decoupled}; learning rates are $5\times 10^{-6}$ and $2\times 10^{-4}$ separately for encoders and centroid embeddings; $\lambda$ in Eq.~(\ref{eq:weighted_sum_loss}) is set to 0.05 for $M=48/32/24$, 0.07 for $M=16$, 0.1 for $M=12$, 0.2 for $M=8$, and 0.3 for $M=4$; batch sizes are separately set to 1024 and 256 for passage and document ranking. 
In the second stage where dynamic hard negatives are used, the optimizer is AdamW~\cite{loshchilov2017decoupled}; learning rates are $2\times 10^{-6}$ and $2\times 10^{-5}$ separately for encoders and centroid embeddings; batch sizes are  set to 128.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.6\textwidth]{figures/model}
%    \caption{Discretizing dense representations. }
%    \label{fig:pgt}
%\end{figure}







==> tables/category.tex <==

\bgroup
\def\arraystretch{1.5}  % for the vertical padding, 1 is the default, change whatever you need
\setlength{\tabcolsep}{0.5em} % for the horizontal padding

\begin{table*}[t]
\centering
\caption{Dense Retrieval Models}
\scalebox{0.75}{
\begin{tabular}{l | c  c} 
\toprule
 & \textbf{Discrete Query Rep.} & \textbf{Continuous Query Rep.} \\
 \midrule
 \textbf{Discrete Doc Rep.} & 
 \begin{tabular}[l]{cx{0.3\textwidth}} 
 RepMoT~(Ours) \end{tabular}
  &
 \begin{tabular}[l]{cx{0.3\textwidth}} 
 JPQ~\cite{zhan2021jointly}, RepCONC~\cite{zhan2021learningdr} \end{tabular}  
 \\ 
 \textbf{Continuous Doc Rep.} & &
 \begin{tabular}[l]{p{0.45\textwidth}} DPR~\cite{karpukhin2020dense}, ANCE~\cite{xiong2021approximate}, ADORE~\cite{zhan2021optimizing}, RocketQA~\cite{qu2021rocketqa}, TAS-B~\cite{hofstatter2021efficiently}, CLEAR~\cite{gao2020complementing}
 \end{tabular}
 \\
\bottomrule
\end{tabular}}
\end{table*}

\egroup
